Extending the OmpSs-2 Programming Model for Hybrid Quantum-Classical Programming

The OmpSs-2 programming model is used in HPC programs to parallelize code and offload code to accelerators. In this work, we extend the offloading capability to quantum computers. We explain the necessary changes to the Clang compiler and the Nanos6 runtime, which are both part of OmpSs-2. In addition, we develop a simulator that simulates a quantum computer in the network and receives the jobs offloaded by the runtime. Four detailed examples show how our programming model can be used to write hybrid quantum-classical software. The examples are random number generation, a parameter scan using the mean-field ansatz, a variational algorithm using this ansatz, and handwritten digit recognition using a hybrid convolutional neural network.

==> implementation_details.tex <==
\section{Implementation Details}
\todo[inline]{Describe some aspects of implementation in more detail: Implementation of Quantum Simulator, communication with quantum device, parameter handling...}
